Reachability and Coverage Planning for Connected Agents: Extended Version

Motivated by the increasing appeal of robots in information-gathering missions, we study multi-agent path planning problems in which the agents must remain interconnected. We model an area by a topological graph specifying the movement and the connectivity constraints of the agents. We study the theoretical complexity of the reachability and the coverage problems of a fleet of connected agents on various classes of topological graphs. We establish the complexity of these problems on known classes, and introduce a new class called sight-moveable graphs which admit efficient algorithms.

==> results_tab.tex <==
\begin{figure*}[!t]
    \begin{tabular}{l|c|c||c|c}
      \multirow{2}{*}{Topological Graph - Problem} & \pbReach{} & \pbCoverage{} & \pbBReach{} & \pbBCoverage{}
      \\
      & (Def. \ref{def:pb:reach}) & (Def. \ref{def:pb:cover}) &
      (Def. \ref{def:pb:breach}) & (Def. \ref{def:pb:bcover}) \\\hline
      
      Directed & \multirow{2}{*}{\shortstack{PSPACE-complete \\ (Th.
      \ref{th:dir:compl:reach})}} & \multirow{2}{*}{\shortstack{PSPACE-complete
      \\ (Th. \ref{th:dir:compl:cover})}} & \multirow{6}{*}{NP-complete
      \nocite{Hollinger:2012}} & \multirow{10}{*}{\shortstack{NP-complete \\ $d =
      1$ (Th. \ref{th:cc:compl:bcover})}} \\
      (Def. \ref{def:topo:dir}) & & & & \\\cline{1-3}

  
      Neighbor-Communicable & \multirow{4}{*}{PSPACE-complete \nocite{dblp:conf/aaai/tateobrab18}}
      & \multirow{2}{*}{\shortstack{PSPACE-complete \\ (Th. \ref{th:nc:compl:cover})}} & &
      % \\
      % \begin{tikzpicture}
      %   \node (s) at (0, 0) {};
      %   \node (t) at (3, 0) {};
      %   \draw[->] (s) -- (t);
      %   \draw[communication,tobehere] (s) edge[bend right=20] (t);
      % \end{tikzpicture} & & & & 
      \\
      (Def. \ref{def:topo:nc}) & & & & \\\cline{1-1}\cline{3-3}


      \multirow{2}{*}{Undirected} & & \multirow{2}{*}{?} & & % \\  
      % \begin{tikzpicture}
      %   \node (s) at (0, 0) {};
      %   \node (t) at (3, 0) {};
      %   \draw[-] (s) -- (t);
      %   \draw[communication,tobehere] (s) edge[bend right=20] (t);
      % \end{tikzpicture} & & & &
      \\
       & & & & \\\cline{1-4}
      
      Sight-Moveable &
      \multirow{4}{*}{\shortstack{in LOGSPACE \\ (Prop. \ref{prop:sm:ub:reach})}} &
      \multirow{4}{*}{\shortstack{in LOGSPACE \\ (Prop. \ref{prop:sm:ub:cover})}} &
      NP-complete &
      % \\ 
      % \begin{tikzpicture}
      %   \node (s) at (0, 0) {};
      %   \node (t) at (3, 0) {};
      %   \node (1) at (1, -0.5) {};
      %   \node (2) at (2, -0.5) {};
      %   \draw[communication] (s) -- (t);
      %   \draw[-, tobehere] (s) -- (1);
      %   \draw[-, tobehere] (1) -- (2);
      %   \draw[-, tobehere] (2) -- (t);
      %   \draw[communication, tobehere] (s) edge[bend right=10] (1);
      %   \draw[communication, tobehere] (1) edge[bend right=10] (2);
      %   \draw[communication, tobehere] (2) edge[bend right=10] (t);
      %   \draw[communication, tobehere] (1) edge[bend right=4] (t);
      %   \draw[communication, tobehere] (s) edge[bend right=4] (2);
      % \end{tikzpicture} & & &$(k=3)$  &
       \\ % \hline
       (Def. \ref{def:topo:sm}) & & & $\ell>2$ (Th. \ref{th:sm:compl:breach}) &
       \\\cline{1-1}\cline{4-4}

      
       Complete Communication & & & \multirow{2}{*}{\shortstack{in LOGSPACE\\
       Prop. \ref{prop:cc:ub:breach}}} & \\
       (Def. \ref{def:topo:compl}) & & & &
      % \\
      %  \begin{tikzpicture}
      %  \node (1) at (0.5, 0) {};
      %  \node (2) at (2.5, 0) {};
      %  \node (3) at (1, -0.5) {};
      %  \node (4) at (2, -0.5) {};
      %  \node (5) at (1.5, 0.5) {};
      %  \foreach \x in {1, ..., 5} {
      %  \foreach \y in {1, ..., 5} {
      %  	\draw[communication,tobehere] (\x) -- (\y);
      %  }}
      %  \end{tikzpicture} & & &  & ($d=1$) \\ 
    \end{tabular}
    \caption{Complexity results (with $d$ and $\ell$ the fixed number of agents and steps, respectively).}
    \label{fig:results}
  \end{figure*}
